RGBD Based Dimensional Decomposition Residual Network for 3D Semantic Scene Completion

RGB images differentiate from depth images as they carry more details about the color and texture information, which can be utilized as a vital complementary to depth for boosting the performance of 3D semantic scene completion (SSC). SSC is composed of 3D shape completion (SC) and semantic scene labeling while most of the existing methods use depth as the sole input which causes the performance bottleneck. Moreover, the state-of-the-art methods employ 3D CNNs which have cumbersome networks and tremendous parameters. We introduce a light-weight Dimensional Decomposition Residual network (DDR) for 3D dense prediction tasks. The novel factorized convolution layer is effective for reducing the network parameters, and the proposed multi-scale fusion mechanism for depth and color image can improve the completion and segmentation accuracy simultaneously. Our method demonstrates excellent performance on two public datasets. Compared with the latest method SSCNet, we achieve 5.9% gains in SC-IoU and 5.7% gains in SSC-IOU, albeit with only 21% network parameters and 16.6% FLOPs employed compared with that of SSCNet.

==> figs/selfParams.tex <==
%-------------------------------------------------------------------------
\begin{table}[t]
\begin{center}
\scalebox {0.8}
{
\begin{tabular} {l|c|r| r} 
\hline
Method 								& Params/k & FLOPs/G & performance\\ \hline
rgbd-3dconv 		 			& 2.0M & 277.7  & \\
rgbd-ddr-block(none-bottle)    & 431.0  &  63.3 & \\
single-ddr-block \& ddr-aspp 	& 155.0  & 20.6  & \\ 
rgbd-ddr-block fusion \& ddr-aspp 	& 195.0  & 27.2  & \\ 
% ours-rgbd-ddr-block \& ddr-aspp 	& 188.0  & 26.7  & \\ 
\hline
\end{tabular}
}
\label{tab:selfParamsFLOPs}
\end{center}
\caption{Params and FLOPs.}
\end{table}
%-------------------------------------------------------------------------

==> figs/subNYUCADrgbd.tex <==
\begin{figure*}[t]
\begin{center}
{\includegraphics[width=0.99\linewidth]{images/sub-viz-NYUCAD-RGBD.pdf}}
\end{center}
\caption{Qualitative results on NYUCAD. From left to right: Input RGB-D image,
ground truth, results obtained by our approach, and results obtained by SSCNet~\cite{song2017_SSCNet}. 
Overall, our completed semantic 3D scenes are less cluttered and show a higher voxel class accuracy compared to SSCNet.}
\label{fig:subNYUCADrgbd}
\end{figure*}

==> figs/subNYUCADrgbvsdepth.tex <==
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=0.99\linewidth]{images/sub-viz-NYUCAD-depthvsrgb.pdf}
\end{center}
\caption{Results of single branch of RGB or Depth  image as input of feature extractor.}
\label{fig:subNYUCADrgbvsdepth}
\end{figure*}

==> figs/subtabddr.tex <==
\begin{table}[!htbp]
\begin{center}
\scalebox{0.99}
{
\begin{tabular}{c|c}
\hline
Operation      & Kernel, Channels, Dilation \\ \hline
PWConv & $1\times 1\times 1, w/4, 1$ \\
DDRConv       & $1\times 1\times k, w/4, d$ \\
DDRConv       & $1\times k\times 1, w/4, d$ \\
DDRConv       & $k\times 1\times 1, w/4, d$ \\
PWConv & $1\times 1\times 1, w, 1$ \\ \hline
\end{tabular}
}

\label{tab:ConvInDdr3d}
\end{center}
\caption{Details of the tipical DDR\_3D($k,w,d$). $k$ is the kernel size, $w$ is the channels of the output feature maps and $d$ is the dilation rate.}
\end{table}

==> figs/subtabnetwork.tex <==
\begin{table*}[ht]  % !htbp
% \begin{table*}[H]  % !htbp
\begin{center}
\scalebox{0.9}
{
% Please add the following required packages to your document preamble:


\begin{tabular}{c|c|c|c|c}
\hline \hline
Module                             & Operation        & Size                      & \multicolumn{2}{c}{Kernel, Channels, Dilation}                        \\ \hline \hline
Input                              &                  & $640\times 480$           & Color Image                       & Depth Image                       \\ \hline \hline
\multirow{8}{*}{Feature extractor} & PWConv           & $640\times 480$           & conv($1\times 1,8,1$)                       & conv($1\times 1,8,1$)                   \\ \cline{2-5} 
                                   & DDR              & $640\times 480$           & DDR\_2d(3,8,1)                      & DDR\_2d(3,8,1)                  \\ \cline{2-5} 
                                   & DDR              & $640\times 480$           & DDR\_2d(3,8,1)                      & DDR\_2d(3,8,1)                  \\ \cline{2-5} 
                                   & projection layer & $240\times 144\times 240$ & projection                        & projection                        \\ \cline{2-5} 
                                   & Down-sample      & $120\times 72\times 120$  & {[}pooling(8), conv($1\times 1\times 1, 8, 1$){]}   & {[}pooling(8), conv($1\times 1\times 1, 8, 1$){]}   \\ \cline{2-5} 
                                   & DDR              & $120\times 72\times 120$  & DDR\_3d(3,16)                     & DDR\_3d(3,16)                     \\ \cline{2-5} 
                                   & Down-sample      & $60\times 36\times 60$    & {[}pooling(16), conv($1\times 1\times 1, 48, 1$){]} & {[}pooling(16), conv($1\times 1\times 1, 48, 1$){]} \\ \cline{2-5} 
                                   & DDR              & $60\times 36\times 60$    & DDR\_3d(3,64,1)                     & DDR\_3d(3,64,1)                 \\ \hline \hline
\multirow{3}{*}{Feature fusion}    & DDR              & $60\times 36\times 60$    & DDR\_3d(3,64,2)                   & DDR\_3d(3,64,2)                   \\ \cline{2-5} 
                                   & DDR              & $60\times 36\times 60$    & DDR\_3d(3,64,3)                   & DDR\_3d(3,64,3)                   \\ \cline{2-5} 
                                   & DDR              & $60\times 36\times 60$    & DDR\_3d(3,64,5)                   & DDR\_3d(3,64,5)                   \\ \hline \hline
\multirow{5}{*}{LW-ASPP}           & PWConv           & $60\times 36\times 60$    & \multicolumn{2}{c}{conv$(1\times 1\times 1, 64, 1)$}                                   \\ \cline{2-5} 
                                   & DDR              & $60\times 36\times 60$    & \multicolumn{2}{c}{DDR\_3d(3,64,3)}                                  \\ \cline{2-5} 
                                   & DDR              & $60\times 36\times 60$    & \multicolumn{2}{c}{DDR\_3d(3,64,6)}                                  \\ \cline{2-5} 
                                   & DDR              & $60\times 36\times 60$    & \multicolumn{2}{c}{DDR\_3d(3,64,9)}                                  \\ \cline{2-5} 
                                   & AvgPooling       & $60\times 36\times 60$    & \multicolumn{2}{c}{AvgPooling}                                       \\ \hline \hline
\multirow{3}{*}{Output}            & PWConv           & $60\times 36\times 60$    & \multicolumn{2}{c}{conv$(1\times 1\times 1, 128, 1)$}                                  \\ \cline{2-5} 
                                   & PWConv           & $60\times 36\times 60$    & \multicolumn{2}{c}{conv($1\times 1\times 1, 128, 1$)}                                  \\ \cline{2-5} 
                                   & PWConv           & $60\times 36\times 60$    & \multicolumn{2}{c}{conv($1\times 1\times 1, 12, 1$)}                                   \\ \hline \hline
\end{tabular}

}

\label{tab:ConvInLwssc}

\end{center}
\caption{ The detail of the proposed network architecture.}
% Table 1. Architectures for ImageNet. Building blocks are shown in brackets (see also Fig. 5), with the numbers of blocks stacked. Downsampling is performed by conv3 1, conv4 1, and conv5 1 with a stride of 2.
\vspace{-8cm}
\end{table*}
